Template-based Program Synthesis using Stellens\"atze

Template-based synthesis, also known as sketching, is a localized approach to program synthesis in which the programmer provides not only a specification, but also a high-level ``sketch'' of the program. The sketch is basically a partial program that models the general intuition of the programmer, while leaving the low-level details as unimplemented ``holes''. The role of the synthesis engine is then to fill in these holes such that the completed program satisfies the desired specification. In this work, we focus on template-based synthesis of polynomial imperative programs with real variables, i.e.~imperative programs in which all expressions appearing in assignments, conditions and guards are polynomials over program variables. While this problem can be solved in a sound and complete manner by a reduction to the first-order theory of the reals, the resulting formulas will contain a quantifier alternation and are extremely hard for modern SMT solvers, even when considering toy programs with a handful of lines. Moreover, the classical algorithms for quantifier elimination are notoriously unscalable and not at all applicable to this use-case. In contrast, our main contribution is an algorithm, based on several well-known theorems in polyhedral and real algebraic geometry, namely Putinar's Positivstellensatz, the Real Nullstellensatz, Handelman's Theorem and Farkas' Lemma, which sidesteps the quantifier elimination difficulty and reduces the problem directly to Quadratic Programming (QP). Alternatively, one can view our algorithm as an efficient way of eliminating quantifiers in the particular formulas that appear in the synthesis problem. The resulting QP instances can then be handled quite easily by SMT solvers. Notably, our reduction to QP is sound and semi-complete, i.e.~it is complete if polynomials of a sufficiently high degree are used in the templates...

==> chapters/conclusion_and_future_work.tex <==
\section{Conclusions and Future Work}\label{section_conlcusions}

==> chapters/intro.tex <==
\section{Introduction}
An imperative program is a sequence of instructions in a programming language that manipulate the memory to solve a problem. The task of writing the program is usually done by a programmer who first comes up with a high-level idea for the algorithm, and then they implement their algorithm by writing a program. Synthesis makes the later part easier; given logical specification for the program, we can synthesize a program that satisfies those specifications. Syntax-Guided Synthesis problem (SyGuS) module theory $T$ is a general synthesis problem of a function $f$ given \textit{semantic constraint} as a formula built from symbols in theory $T$ and $f$, and \textit{syntactic constraint} given as a (possibly infinite) set of expressions from $T$ specified using a context-free grammar. 

In this paper, we focus on Syntax-Guided program synthesis problem module theory of Polynomial Arithmetic (over reals).

The treatment here generalises the methods for program synthesis used in \cite{srivastava2013template} for linear programs to polynomial programs. Our main tools include the use of classical theorems from Real Algebraic Geoemtry \cite{bochnak2013real} like Handelman's Theorem (Thoerem \ref{thm:handel}), Putinar’s Positivstellensatz (Theorem \ref{theorem_put_pos}) and Real Nullstellensatz (Theorem \ref{theorem_real}). We provide with a sound and semi-complete synthesis algorithm for polynomial programs.

\textbf{Outline of the paper:} In Section \ref{sec_problem_statement}, we defined the notions of programs, semantics and templates. We also give a mathematically precise formulation of the problem in terms of constraint pairs. In Section \ref{section:toolkit}, we presented classical theorems from Real Algebraic Geometry required for design of the synthesis algorithm. We also presented Theorem \ref{technical_tool_1} which is a new mathematical contribution from this paper. In Section \ref{synthesis_algo}, we presented our synthesis algorithm along with proving it's soundness and semi-completeness. Finally in Section \ref{secion_proof_of_concept} we presented a proof of our proposed concept by providing experimentation results on small programs. 
